Checking Robustness against TSO

We present algorithms for checking and enforcing robustness of concurrent programs against the Total Store Ordering (TSO) memory model. A program is robust if all its TSO computations correspond to computations under the Sequential Consistency (SC) semantics. We provide a complete characterization of non-robustness in terms of so-called attacks: a restricted form of (harmful) out-of-program-order executions. Then, we show that detecting attacks can be parallelized, and can be solved using state reachability queries under SC semantics in a suitably instrumented program obtained by a linear size source-to-source translation. Importantly, the construction is valid for an arbitrary number of addresses and an arbitrary number of parallel threads, and it is independent from the data domain and from the size of store buffers in the TSO semantics. In particular, when the data domain is finite and the number of addresses is fixed, we obtain decidability and complexity results for robustness, even for an arbitrary number of threads. As a second contribution, we provide an algorithm for computing an optimal set of fences that enforce robustness. We consider two criteria of optimality: minimization of program size and maximization of its performance. The algorithms we define are implemented, and we successfully applied them to analyzing and correcting several concurrent algorithms.

==> figures/scwitness.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[node distance=1.8cm]

  \node(inv){$\sigma =$ };
  \node(bul)[right of=inv,node distance=2.2cm,color=gray]{$\issueact_{\attacklocalstore}\cdot \attacklocalstore$};
  \node(ld)[right of=bul,node distance=2.3cm,color=red] {$\attackload$};
  \node(winv)[right of=ld,node distance=1.3cm] {};

  %\node(inv0)[below of=inv,node distance=1cm]{};
  %\node(inv2)[left of=inv0,node distance=0.2cm]{Attacker




  \draw[-, very thick] (inv)edge node[above]{$\tau_1$} (bul);
  \draw[-, very thick] (bul)edge node[above]{$\tau_2'$} (ld);
  \draw[-, very thick,color=blue] (ld)edge
					node[above,color=black]{$\tau_3$}(winv);



\end{tikzpicture}
\caption{SC computation of an instrumented program $\aprog_{\attack}$ representing a TSO witness for attack $\attack$.
The delayed stores are replaced by stores to addresses that are local (indicated in gray) to the attacker.
All these stores are contained in $\tau_2'$. \rfm{We can improve the figure as follows. 
The above line denotes the writes to main memory. When the attacker starts delaying stores,
we make a second line below this one that represents the auxiliary variables. The stores act here, the loads that do not prefetch act on top. But we need to get across well the idea that the one line is for global memory and the second is for attacker auxiliaries.}
\label{Figure:SCWitness}}
\end{figure}

